Mockingbird: Defending Against Deep-Learning-Based Website Fingerprinting Attacks with Adversarial Traces

Website Fingerprinting (WF) is a type of traffic analysis attack that enables a local passive eavesdropper to infer the victim's activity, even when the traffic is protected by a VPN or an anonymity system like Tor. Leveraging a deep-learning classifier, a WF attacker can gain over 98% accuracy on Tor traffic. In this paper, we explore a novel defense, Mockingbird, based on the idea of adversarial examples that have been shown to undermine machine-learning classifiers in other domains. Since the attacker gets to design and train his attack classifier based on the defense, we first demonstrate that at a straightforward technique for generating adversarial-example based traces fails to protect against an attacker using adversarial training for robust classification. We then propose Mockingbird, a technique for generating traces that resists adversarial training by moving randomly in the space of viable traces and not following more predictable gradients. The technique drops the accuracy of the state-of-the-art attack hardened with adversarial training from 98% to 42-58% while incurring only 58% bandwidth overhead. The attack accuracy is generally lower than state-of-the-art defenses, and much lower when considering Top-2 accuracy, while incurring lower bandwidth overheads.

==> 3_1_back_onion_sites.tex <==
\subsection{Onion Sites}\label{onion-sites}
%\todo[inline]{MI:Do we need to put this here, may be in discussion}
An onion site, formerly known as a {\em hidden service}, is an anonymized service provided through Tor. The locations and the IP addresses of onion servers are not known by Tor nodes nor their clients. Onion sites provide various kinds of services such as web publishing, messaging, and chat. These sites are particular interesting in that the services they provide are often very sensitive in nature.

Recent studies~\cite{unique-ccs2017,Kwon2015} have shown that onion sites' traffic can be easily distinguished from other types of Tor traffic. Therefore, the adversary can easily filter out the onion sites' traffic from the rest of Tor traffic and specifically target these sites in a WF attack. Given that the number of onion sites is very small compared to that of the regular Web, the WF attacker is dealing with a small open world. Thus, the threat of WF against onion sites is particularly serious.  As such this is a strong motivational force for the timely development of reliably effective WF defenses.

%\todo[inline]{redundant information already explained in WF Defenses}
%Fortunately, onion sites are typically more concerned than regular websites on the anonymity of their users, and so they may be more willing to contribute in defense against WF attacks. Cherubin et al.~\cite{Cherubin2017} leveraged this understanding in their ALPaCa defense, which is deployed by the website owner. Their defense was effective at reducing the accuracy of state-of-the-art attacks from 70\% down to 10-40\%, but results in a relatively high latency overhead of 40-60\%. 


%\todo[inline]{This section seems to imply adversarial examples are most appropriately applied onion sites, and not necessarily general Tor. Is it necessary that the server owner be responsible for generating a profile of their site?}

%We propose to extend this approach by creating adversarial examples based on the server's knowledge of its own page profile. Creating adversarial examples for onion sites can then be less challenging. The onion server can generate the adversarial examples for its traffic and ship them to the client. Both, the client and server, follow that traffic pattern during the transmission. 



==> 6_1_challenges.tex <==
\subsection{Deployment Challenges}
\label{challenges}
Generating adversarial examples for WF defense is different than that of other domains such as computer vision or voice recognition. The main challenges we face in crafting adversarial examples for web traffic traces are as follows:
%In contrast to their typical applications, adversarial examples in WF must be generated from Web traffic traces. This is different than adversarial examples in other fields such as image classification, voice recognition, and text classification, and thus makes the use of existing techniques in generating adversarial examples ineffective for WF defense. The main challenges we face in crafting adversarial examples for web traffic traces are as follows:

\paragraphX{\textbf{No Packet Dropping, only Insertion.}} Perturbation to traffic traces can be done only through the sending of the dummy packets. Dropping real packets to perturb the traffic trace is undesirable as dropped packets will need to be re-queued before subsequent packets, causing time delays. %not recommended due to network re-transmissions that lead to higher bandwidth and latency overhead, and harming the user's experience. 
To overcome this challenge, we introduce constraints in our algorithm to insure that the packet burst sizes are only ever increased (see~Section~\ref{genadvtraces}).
  
\paragraphX{\textbf{Two Parties are Involved.}} Traffic traces are a combination of download and upload streams. Neither the client nor the server has a full control of both streams. Therefore, the WF defense has two elements to control both sides of the traffic: the client side and a bridge in the network. This dynamic imposes unique restrictions on the implementation of our design that do no exist in other domains for adversarial examples. %Generating the adversarial traces in the burst level enables us to generate them in the server and send them to the client. 
  
\paragraphX{\textbf{Crafting Adversarial Examples on the Fly.}} To craft the adversarial examples from traffic traces, we have to deal with the transmission of packets. Ideally, the traffic trace should be captured packet by packet and the adversarial examples should be generated in real time so that we can send and receive packets simultaneously. In addition, as the entire trace is not accessible to the algorithm during the application of the defense, the adversarial examples should be generated on the fly. Furthermore, the client must use a pre-trained detector that models the attacker when generating the adversarial traces. These detectors are deep-learning classification models, and consequently require significant computing capacity to generate traces for each site visit. %Such a capability might not practical to assume, so we require an alternate way to make this defense work in the Tor network (see Section~\ref{alternate_deploy}).
%To tackle this challenge, we propose to generate adversarial traces at the burst-level rather than the cell-level. Both the client and the bridge will follow the agreed traffic pattern in their communication.

==> appen_B.tex <==
\section{\textbf{Weaker Surrogate Network}}%\label{surrogate}
\label{weak_surrogate}
%\vspace{-0.9cm}
\begin{figure}[ht]
\centering
  \includegraphics[scale=0.5]{figures/W_HD_Top_K.png}
  \caption{\textbf{Weak Detector:} Half-duplex Performance. $x$-axis represents the Top-$k$ where $k$=$1....10$ and $y$-axis represents the attack accuracy.}
  \label{fig:weak_network_hd}
\end{figure}
%\vspace{-0.5cm}
One of the concerns of generating adversarial traces with respect to a powerful detector is that the powerful detector today can be obsolete tomorrow and a more powerful attack might make this defense ineffective. To address this concern, we generate adversarial traces with respect to a very week detector. However, we still use a powerful attack model DF for adversarial training. The architecture of this detector is shown in Table~\ref{cnn_modelarch}. We only show the experimental results for half-duplex dataset. Our results show that our defense remain effective even though we use a weak surrogate network. The bandwidth overheads for Case I and Case II is 62\% and 73\%, respectively. The Top-1 attack accuracy is 35\% and 29\% for Case I and Case II, respectively. We can see the Top-1 to Top-10 accuracy in Figure~\ref{fig:weak_network_hd}. Top-10 accuracy for both Case I and Case II is lower than 90\%. In particular, Top-10 accuracies for both Case I and Case II are 86\% and 81\%, respectively.  



==> appen_C.tex <==
%\subsection{Analysis of Top-$k$ Accuracy}
%\label{top_k_analysis}
%\vspace{-0.9cm}
%\vspace{-0.9cm}

\begin{figure}[t!]
\centering
  \input{figures/top_k_all}
  \caption{\textbf{Top-$k$ Accuracy:} full-duplex and half-duplex. $x$-axis represents the Top-$k$ where $k$=$1....10$ and $y$-axis represents the attack accuracy.} %Red and Green solid line represents the results for full-duplex dataset and dashed line represents the results for half-duplex dataset.}
  \label{fig:top_k_10}
\end{figure}


%\vspace{-0.5cm}
%\begin{figure}[ht!]
%\centering
%  \includegraphics[scale=0.55]{figures/HDFD_BOX_Total.png}
%  \caption{Total Number Target Changes for both HD and FD dataset.}
%  \label{fig:total_target_change}
%\end{figure}


\begin{figure}[t!]
\centering
  \includegraphics[scale=0.50]{figures/fd_hd_box_5.png}
  \caption{\textbf{Site-5:} Number of Target Changes in both HD and FD.}
  \vskip -0.3cm
  \label{fig:site_5_total_target_change}
\end{figure}

We can see from Figure~\ref{fig:top_k_10} that \system~ can limit the Top-10 accuracies of full-duplex (FD) data to 84\% and 92\% for Case I and Case II, respectively. For half-duplex (HD), Top-10 accuracies are 86\% and 80\% for Case I and Case II. These set of results show that \system~is better to limit the Top-$k$ accuracy to a significant degree than that of W-T and WTF-PAD defenses. \system~is doing such a good job because of the way it picks a target trace. Robust randomness to pick a target trace and the role of detector enables \system~to be resistant to Top-$k$ accuracy. We mention in our defense design that \system~picks a new target trace each time detector indicates the adversarial sample confidence is not lower than a threshold value. In this way, the final generated adversarial trace is a result of picking multiple target trace.

%We visualize the total number of changes of the target trace for both full-duplex and half-duplex datasets in a box-plot in Figure~\ref{fig:total_target_change}. 
%For FD Case I, the median, $1_{st}$ quartile, $3_{rd}$ quartile, lower whisker, and upper whisker are 400, 248, 704, 57, and 1193, respectively. For Case II, the median, $1_{st}$ quartile, $3_{rd}$ quartile, lower whisker, and upper whisker are 522, 285, 843, 65, and 1546, respectively. For HD Case I, the median, $1_{st}$ quartile, $3_{rd}$ quartile, lower whisker, and upper whisker are 609, 419, 744, 85, and 1218, respectively. For Case II, the median, $1_{st}$ quartile, $3_{rd}$ quartile, lower whisker, and upper whisker are 360, 174, 617, 23, and 1026, respectively.

For a better understanding of the target change, we analyse site-5. In our dataset, FD site 5 and HD site 5 is the same. We can see the box-plot of the number of target change in Figure~\ref{fig:site_5_total_target_change}. The median number of target changes for FD are 77 and 74 for Case I and Case II, respectively. For HD, median number of target changes are 2 and 1 for Case I and Case II, respectively.


% FD Case I: 1Q, 3Q, Lower Whisker, upper whisker: 9, 128, 0, 304

% FD Case II: 1Q, 3Q, Lower Whisker, upper whisker: 33, 147, 0, 318

% HD Case I: 1Q, 3Q, Lower Whisker, upper whisker: 1, 4, 0, 7

% HD Case II: 1Q, 3Q, Lower Whisker, upper whisker: 0, 2, 0, 5

==> appen_attack_Scenerios.tex <==

\section{Scenarios of Existing Methods}
\label{failed_carlini}




In order to evaluate the efficacy of the adversarial traces generated by the Carlini and Wagner~\cite{carlini2017towards}  method described in Section~\ref{failed_methods}, we consider two different attack scenarios based on when the defenses are applied. The defense can be applied either after the attack (Without-Adversarial-Training) or before the attack (With-Adversarial-Training). We evaluate both scenarios in the following sections. We use half-duplex (HD) closed-world dataset for these experiments. We explain the pre-processing of the data in Section~\ref{dataset}.




\subsection{SCENARIO I: Without-Adversarial-Training}\label{scenarioI}
In this scenario, we assume that the attacker has trained its classifier on the traces that have not been defended. We assume that the attacker is not aware of a defense in place. Such a scenario can be valid in the case that we have an attacker that does not target any specific client and his goal is to identify the behavior of large number of users, but some of the clients may use some defense to protect their traffic. Here, the attacker is not aware of the defense or his goal is to monitor the majority of the clients.

For this scenario, we first train a classifier on our undefended traces and then we generate the adversarial traces. We examine the efficacy of the generated samples by testing them against the trained attacker model.




In our evaluation we break the data into two sets, {\em Adv Set}, and {\em Detector Set}, each set has 83 classes with 360 instances each. The attacker trains the classifier on the Detector Set. The traces in Detector Set are not protected by any defenses. The WF attacks that we apply on the Adv Set are the DF and CUMUL attacks. We chose DF attack as a state-of-the-art WF attack representing Deep Learning WF attacks, and CUMUL attack as the representative of the traditional machine learning algorithms. CUMUL attack uses SVM classifier and has high performance compared to other tradition WF attacks~\cite{sirinamDF}. 



We apply the method described in~\ref{failed_methods} to generate adversarial traces from the traces in Adv Set, we call these traces in our evaluation as Adversarial Traces. To generate Adversarial Traces, we use our Simple CNN as the target model (F) and the adversarial traces will be generated based on simple CNN. The architecture of our simple CNN is shown in Table~\ref{cnn_modelarch}. 

\input{tables/simple_CNN.tex}
\input{tables/undefended_traces.tex}


Table~\ref{attacker-first} shows the results of our evaluations. According to the table, Adversarial Traces add 62\% bandwidth overhead. Adversarial Traces generated for Simple CNN can confound the target model 98\% of the times. In addition, the accuracy of DF and CUMUL attacks are 3\% and 31\%. This means that Adversarial Traces generated based on a target model with Simple CNN architecture, can be highly transferable to other machine learning models. Almost all the adversarial traces generated by Simple CNN can confound DF attack, which is also a deep learning model. The results show that the adversarial traces are more transferable to DNN model than traditional machine learning models.   


\subsection{SCENARIO II: With-Adversarial-Training}\label{scenarioII}

\input{tables/defended_traces.tex}


In this scenario, we assume that the attacker knows that the client is using some sort of defense mechanisms to protect her traffic. The attacker then collects the traces protected by the same method as the client and trains his classifier with those traces. In this scenario, the training set and testing set are both traces protected by the same WF defense method. This scenario is more realistic because it has been shown that the effectiveness of the WF attacks defends on the attacker's knowledge of the clients~\cite{marc-css-2014}. Moreover, once a defense is deployed it is supposed to be accessible for all the users and used by all the users. Therefore, the attacker can also use  the same defense as other clients. 


For evaluation in this scenario, we protect the traces in Adv Set by Adversarial Traces (described in Section~\ref{failed_methods} using a target model with the architecture in Table~\ref{cnn_modelarch}). Then we train the WF attacks, Simple CNN, DF, and CUMUL attacks, on 90\% defended traces and test them with the remaining 10\% of defended traces. 

To generate Adversarial Traces, we train a target model with the same architecture as Simple CNN with the traces in Detector Set and used in generating Adversarial Traces on Adv Set. The results of the evaluation in this scenario are shown in Table~\ref{defender-first}. As shown in the table, even when adversarial traces are generated based on a target model with similar architecture as Simple CNN, they are highly detectable on Simple CNN as we train Simple CNN on the adversarial traces, and its accuracy is 91\%. Moreover, DF and CUMUL attacks can also detect the adversarial traces with high accuracy, 97\% and 91\%, respectively. This means that generated adversarial traces are ineffective when the adversary adopts the technique of adversarial training. Generating the adversarial traces works like a data augmentation technique in this case. If the attacker is trained on them, the attacker will detect them correctly. This highlights the necessity of the creation of a new adversarial example generation technique designed specifically for WF.

==> extras/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> extras/README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> extras/ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> extras/ccs-template.tex <==


\begin{document}
\title{Template for ACM CCS} % TODO: replace with your title

\begin{abstract}
Your abstract should go here. You will also need to upload a plain-text abstract into the web submission form.
\end{abstract}

% TODO: replace this section with code generated by the tool at https://dl.acm.org/ccs.cfm
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002978.10003029.10011703</concept_id>
<concept_desc>Security and privacy~Usability in security and privacy</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc{Security and privacy~Use https://dl.acm.org/ccs.cfm to generate actual concepts section for your paper}
% -- end of section to replace with generated code

\keywords{template; formatting; pickling} % TODO: replace with your keywords

\maketitle

\input{ccs-body} % TODO: replace with your brilliant paper!

\bibliographystyle{ACM-Reference-Format}
\bibliography{ccs-sample}

\end{document}


==> extras/cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> tables/DFasDetector.tex <==
\begin{table*}[tbp]
\centering

\caption{\textbf{White-Box.} Evaluation of \system~against DF, AWF, CUMUL, $k$-FP, and $k$-NN Attacks \& Comparison against WTF-PAD and W-T Defenses. \textbf{S$\times$I}: Sites$\times$Instances, \textbf{BWO}: Bandwidth Overhead, \textbf{FD}: Full-Duplex, \textbf{HD}: Half-Duplex.}
\begin{tabular}{|llc|c|c|c||ccc|c|c||} 
\hline
\textbf{Cases} & \textbf{Dataset}  & \textbf{S$\times$I} & \textbf{BWO} & \textbf{DF~\cite{sirinamDF}}   & \textbf{AWF~\cite{Rimmer2018}} & \textbf{CUMUL~\cite{cumul}} & \textbf{$k$-FP}~\cite{kfp} & \textbf{$k$-NN}~\cite{Wang2014} & {\bf DF Top-2} \\ 
\hline
& Undefended (FD)   &   95$\times$259   & -            & 0.95 &  0.88 & 0.93 & 0.85 & 0.86 & - \\
& Undefended (HD)  & 83$\times$360 & - & 0.98 & 0.93 & 0.92 & 0.92 & 0.90 & - \\
& WTF-PAD~\cite{wtf-pad} & 95$\times$463 &  0.64 & 0.85 & 0.39 & 0.55 & 0.44 & 0.17  & 0.89  \\ 
& W-T~\cite{Wang2017} & 82$\times$360 & 0.72   & 0.36 & 0.39 & 0.36 & 0.30 & 0.35 & 0.97 \\ 
\hline \hline
\multirow{2}{*}{\textbf{Case I}}& 
\system~(FD) & 95$\times$259 & \textbf{0.56}      & \textbf{0.35}  & \textbf{0.20} &  \textbf{0.232} & \textbf{0.21} & \textbf{0.04} & {\bf 0.51}\\
& \system~(HD) &  83$\times$360 &   \textbf{0.63}     & \textbf{0.35} & \textbf{0.27} &   \textbf{0.300} & 0.33 & \textbf{0.06} & {\bf 0.52}\\
\hline\hline

\multirow{2}{*}{\textbf{Case II}}& \system~(FD) & 95$\times$259 &\textbf{0.56}     &  0.55 & \textbf{0.34} & 0.36  & 0.34 & \textbf{0.06} & {\bf 0.56}\\
& \system~(HD) & 83$\times$360 &   0.73     & \textbf{0.28} & \textbf{0.22} &  \textbf{0.31} & 0.30 & \textbf{0.05} & {\bf 0.43}\\
\hline
\end{tabular}
\label{tab_results_analysis}
\end{table*}

==> tables/input_length.tex <==
\begin{table*}[ht!]
\centering
\caption{Attack Accuracy: Results with respect to input length variation.}
\begin{tabular}{lc|c|c|c} 

\hline
 \multirow{ 2}{*}{$\alpha$}   & \multicolumn{2}{c|}{Case I} & \multicolumn{2}{c}{Case 2} \\ \cline{2-5}
    & 5,000 & 10,000 & 5,000   & 10,000  \\ 
\hline
1         & 0.439  & 0.454  & 0.647 & 0.671 \\
3         & 0.361  & 0.394  & 0.571 & 0.585\\
5         & 0.327  & 0.352  & 0.541 & 0.563\\
7         & 0.345  & 0.351  & 0.513 & 0.565\\
\hline
\label{input_length}                   
\end{tabular}
\end{table*}






==> tables/top_2.tex <==
\begin{table}[!t]
\centering

\caption{Top-2 Accuracy of DF Attack against \system~ and  W-T. \textbf{FD}: Full-duplex, \textbf{HD}: Half-Duplex.}
\begin{tabular}{llc} 
\hline
                 \textbf{Cases} & \textbf{Dataset}  & \textbf{DF~\cite{sirinamDF} Top-2 Accuracy}\\
\hline
& WTF-PAD~\cite{wtf-pad} &  0.897 \\ 
& W-T~\cite{Wang2017} &  0.970 \\ 
\hline \hline
\multirow{2}{*}{\textbf{Case I}}& \system~ (FD) &   \textbf{0.514}      \\
& \system~ (HD) &    \textbf{0.528}   \\
\hline\hline

\multirow{2}{*}{\textbf{Case II}}& \system~ (FD) & \textbf{0.569} \\
& \system~ (HD) &  \textbf{0.432}     \\
\hline
\end{tabular}
\label{tab_top2_acc}
\end{table}

==> top_n_results.tex <==
HD Results

target change for site 5
case 1:
print(zers,ons,twos,threes,fours,fives)
57, 81, 82, 49, 58, 33
case 2:
134, 113, 60, 30, 16, 7

Top 10 acc

Case 1
0.5829986612720183, 0.7500000000797921, 0.8142570281922418, 0.8668005354752343, 0.8962516733601071, 0.9173360107095047, 0.9334002676578251, 0.9437751004813985, 0.9511378849526166, 0.9591700134666729


Case 2
 0.5137215527983874, 0.6740294511378849, 0.7516733601070951, 0.8075635876042776, 0.8390227576176644, 0.8681392235609103, 0.8969210174029452, 0.9109772423025435, 0.9230254350736279, 0.9374163319946452
